Decoupling Features in Hierarchical Propagation for Video Object Segmentation

This paper focuses on developing a more effective method of hierarchical propagation for semi-supervised Video Object Segmentation (VOS). Based on vision transformers, the recently-developed Associating Objects with Transformers (AOT) approach introduces hierarchical propagation into VOS and has shown promising results. The hierarchical propagation can gradually propagate information from past frames to the current frame and transfer the current frame feature from object-agnostic to object-specific. However, the increase of object-specific information will inevitably lead to the loss of object-agnostic visual information in deep propagation layers. To solve such a problem and further facilitate the learning of visual embeddings, this paper proposes a Decoupling Features in Hierarchical Propagation (DeAOT) approach. Firstly, DeAOT decouples the hierarchical propagation of object-agnostic and object-specific embeddings by handling them in two independent branches. Secondly, to compensate for the additional computation from dual-branch propagation, we propose an efficient module for constructing hierarchical propagation, i.e., Gated Propagation Module, which is carefully designed with single-head attention. Extensive experiments show that DeAOT significantly outperforms AOT in both accuracy and efficiency. On YouTube-VOS, DeAOT can achieve 86.0% at 22.4fps and 82.0% at 53.4fps. Without test-time augmentations, we achieve new state-of-the-art performance on four benchmarks, i.e., YouTube-VOS (86.2%), DAVIS 2017 (86.2%), DAVIS 2016 (92.9%), and VOT 2020 (0.622). Project page: https://github.com/z-x-yang/AOT.

==> Figures/ytb.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.99\linewidth]{Sources/more_qua.pdf}

    \caption{Qualitative results on YouTube-VOS~\cite{youtubevos} and DAVIS\cite{davis2017}. R50-DeAOT-L tracks and segments objects well under many challenging scenarios, including similar objects, occlusion, fast motion, etc.}
    \label{fig:youtubevos}

\end{figure}

==> Tables/davis2016.tex <==
\begin{wraptable}[21]{r}{0.45\textwidth}
\begin{center}
\vspace{-6.5mm}
\caption{The quantitative evaluation on the single-object benchmark, DAVIS 2016~\cite{davis2016}.}\label{tab:davis2016}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c c}
\toprule[1.5pt]

\midrule[1pt]
 Method  & Avg & $\mathcal{J}$ & $\mathcal{F}$ & fps \\
\midrule[1pt]
%PReM~\cite{premvos}    & 86.8  & 84.9  & 88.6  & 0.03 \\
% STM~\cite{spacetime}   &  89.3 & 88.7  & 89.9  & 6.3 \\
% CFBI~\cite{cfbi}   & 89.4  & 88.3 & 90.5  & 6.3 \\
CFBI+~\cite{cfbip}   & 89.9  & 88.7 & 91.1  & 5.9 \\
RPCM~\cite{rpcm}  &  90.6  & 87.1  & 94.0 & 5.8 \\
HMMN~\cite{hmmn}   &  90.8 & {89.6}  & {92.0}  & 10.0 \\
STCN~\cite{cheng2021stcn}   &  91.6 & {90.8}  & {92.5}  & 27.2$^\star$ \\
\hline
\hline
AOT-T~\cite{aot}  &  86.8  & 86.1 & 87.4 & {51.4} \\
DeAOT-T  & \textbf{88.9} & \textbf{87.8} & \textbf{89.9} & \textbf{63.5} \\
\hline
AOT-S~\cite{aot}  &  \textbf{89.4}  & \textbf{88.6} & 90.2 & 40.0 \\
DeAOT-S  & {89.3} & {87.6} & \textbf{90.9} & \textbf{49.2} \\
\hline
AOT-B~\cite{aot}  &  89.9  & 88.7 & 91.1 & 29.6 \\
DeAOT-B  & \textbf{91.0} & \textbf{89.4} & \textbf{92.5} & \textbf{40.9} \\
\hline
AOT-L~\cite{aot}  &  {90.4}  & {89.6} & {91.1} & 18.7 \\
DeAOT-L  & \textbf{92.0} & \textbf{90.3} & \textbf{93.7} & \textbf{28.5} \\
\hline
R50-AOT-L~\cite{aot}  &  {91.1}  & {90.1} & {92.1} & 18.0 \\
R50-DeAOT-L  & \textbf{92.3} & \textbf{90.5} & \textbf{94.0} & \textbf{27.0} \\
\hline
SwinB-AOT-L~\cite{aot}  &  {92.0}  & {90.7} & {93.3} & 12.1 \\
SwinB-DeAOT-T  & \textbf{92.9} & \textbf{91.1} & \textbf{94.7} & \textbf{15.4} \\
\bottomrule[1.5pt]

\end{tabular}
\end{center}
\end{wraptable}

==> Tables/full_comparisons.tex <==
\begin{table}[t!]
	\centering
	\caption{Additional quantitative comparison on multi-object benchmarks, YouTube-VOS~\cite{youtubevos} and DAVIS 2017~\cite{davis2017}. $^{*}$: using 600p instead of 480p videos in inference. $^{\ddag}$: timing extrapolated from single-object speed assuming linear scaling in the number of objects. $^{\star}$: recorded on our device.
	}\label{tab:full_comparisons}
	
\begin{subtable}{.54\textwidth}
\centering
\caption{YouTube-VOS}\label{tab:full_youtubevos}
\setlength{\tabcolsep}{3pt}
\small
\vspace{-0.5mm}
\begin{tabular}{lcccccc}
	
\toprule[1.5pt]
            &   &  \multicolumn{2}{c}{Seen}  &    \multicolumn{2}{c}{Unseen} &  \\
\midrule[1pt]
 Methods & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & FPS \\
\midrule[1pt]
\multicolumn{7}{c}{\textit{Validation 2018 Split}} \\
\midrule[1pt]
SAT\pub{CVPR20}~\cite{realtimevos1}  &  63.6  &  67.1  & 70.2  &  55.3  & 61.7 & - \\
AG\pub{CVPR19}~\cite{agame}  &  66.1  &  67.8  &  -  &  60.8  &  - & - \\
PReM\pub{ACCV18}~\cite{premvos}    &  66.9  &  71.4  &  75.9  &  56.5  &  63.7 & 0.17 \\
BoLT\pub{arXiv19}~\cite{boltvos}   &  71.1  &  71.6  &  -  &  64.3  &  - & 0.74 \\

GC\pub{ECCV20}~\cite{realtimevos2}   & 73.2  & 72.6  & 75.6 & 68.9 & 75.7  & - \\
STM\pub{ICCV19}~\cite{spacetime}   &  79.4  &  79.7  &  84.2  &  72.8  &  80.9 & - \\
EGMN\pub{ECCV20}~\cite{EGMN}  &  80.2  &  80.7  &  85.1  &  74.0  &  80.9 & - \\
KMN\pub{ECCV20}~\cite{KMN}  &  81.4  &  81.4  &  85.6  &  75.3  &  83.3 & - \\
CFBI\pub{ECCV20}~\cite{cfbi} &  81.4  &  81.1  & 85.8  & 75.3  & 83.4 & 3.4 \\
LWL\pub{ECCV20}~\cite{LWLVOS} & 81.5  &  80.4  &  84.9  &  76.4  &  84.4 & - \\
SST\pub{CVPR21}~\cite{sstvos} & 81.7  &  81.2  &  -  &  76.0  &  - & - \\
CFBI+\pub{TPAMI21}~\cite{cfbip} &  82.8  &  81.8  & 86.6  & 77.1  & 85.6 & 4.0 \\
HMMN\pub{ICCV21}~\cite{hmmn} & 82.6  &  82.1  &  87.0  &  76.8  &  84.6 & -  \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn} &  83.0  &  81.9  & 86.5  & 77.9  & 85.7 & 8.4$^\star$ \\
RPCM\pub{AAAI22}~\cite{rpcm} &  84.0  &  83.1  & 87.7  & 78.5  & 86.7 & -  \\
\hline
\hline
AOT-T~\cite{aot} & 80.2  &  80.1  & 84.5  & 74.0  & 82.2 & {41.0} \\
DeAOT-T & \textbf{82.0}  &  \textbf{81.6}  & \textbf{86.3}  & \textbf{75.8}  & \textbf{84.2} & \textbf{53.4} \\
\hline
AOT-S~\cite{aot}  & 82.6  &  82.0  & 86.7  & 76.6  & 85.0 & {27.1} \\
DeAOT-S & \textbf{84.0}  &  \textbf{83.3}  & \textbf{88.3}  & \textbf{77.9}  & \textbf{86.6} & \textbf{38.7} \\
\hline
AOT-B~\cite{aot}  & 83.5  &  {82.6}  & 87.5  & {77.7}  & 86.0 & 20.5 \\
DeAOT-B & \textbf{84.6}  &  \textbf{83.9}  & \textbf{88.9}  & \textbf{78.5}  & \textbf{87.0} & \textbf{30.4} \\
\hline
AOT-L~\cite{aot}  & {83.8}  &  {82.9}  & {87.9}  & {77.7}  & {86.5} & 16.0 \\
DeAOT-L & \textbf{84.8}  &  \textbf{84.2}  & \textbf{89.4}  & \textbf{78.6}  & \textbf{87.0} & \textbf{24.7} \\
\hline
R50-AOT-L~\cite{aot}  & {84.1}  &  {83.7}  & {88.5}  & {78.1}  & {86.1} & 14.9 \\
R50-DeAOT-L & \textbf{86.0}  &  \textbf{84.9}  & \textbf{89.9}  & \textbf{80.4}  & \textbf{88.7} & \textbf{22.4} \\
\hline
SwB-AOT-L~\cite{aot}  & {84.5}  &  {84.3}  & {89.3}  & {77.9}  & {86.4} & 9.3 \\
SwB-DeAOT-L & \textbf{86.2}  &  \textbf{85.6}  & \textbf{90.6}  & \textbf{80.0}  & \textbf{88.4} & \textbf{11.9} \\
\midrule[1pt]
\multicolumn{7}{c}{\textit{Validation 2019 Split}} \\
\midrule[1pt]
CFBI\pub{ECCV20}~\cite{cfbi}  &  81.0  &  {80.6}  & {85.1}  & {75.2}  & {83.0} & 3.4  \\
SST\pub{CVPR21}~\cite{sstvos} & 81.8  &  80.9  &  -  &  76.6  &  - & - \\
HMMN\pub{ICCV21}~\cite{hmmn} & 82.5  &  81.7  &  86.1  &  77.3  &  85.0 & - \\
CFBI+\pub{TPAMI21}~\cite{cfbip} &  82.6  &  81.7  & 86.2  & 77.1  & 85.2 & 4.0 \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn}  &  82.7  &  81.1  & 85.4  & 78.2  & 85.9 & 8.4$^\star$ \\
RPCM\pub{AAAI22}~\cite{rpcm} &  83.9  &  82.6  & 86.9  & 79.1  & 87.1 & - \\
\hline
\hline
AOT-T~\cite{aot}  &  79.7  &  79.6  & 83.8  & 73.7  & 81.8 & {41.0} \\
DeAOT-T & \textbf{82.0}  &  \textbf{81.2}  & \textbf{85.6}  & \textbf{76.4}  & \textbf{84.7} & \textbf{53.4} \\
\hline
AOT-S~\cite{aot}  &  82.2 &  81.3  & 85.9  & 76.6  & 84.9 & {27.1} \\
DeAOT-S & \textbf{83.8}  &  \textbf{82.8}  & \textbf{87.5}  & \textbf{78.1}  & \textbf{86.8} & \textbf{38.7} \\
\hline
AOT-B~\cite{aot}  &  83.3 &  {82.4}  & {87.1}  & 77.8  & 86.0 & 20.5 \\
DeAOT-B & \textbf{84.6}  &  \textbf{83.5}  & \textbf{88.3}  & \textbf{79.1}  & \textbf{87.5} & \textbf{30.4} \\
\hline
AOT-L~\cite{aot}  &  {83.7} &  {82.8}  & {87.5}  & {78.0}  & \textbf{86.7} & 16.0 \\
DeAOT-L & \textbf{84.7}  &  \textbf{83.8}  & \textbf{88.8}  & \textbf{79.0}  & \textbf{87.2} & \textbf{24.7} \\
\hline
R50-AOT-L~\cite{aot}  & {84.1}  &  {83.5}  & {88.1}  & \textbf{78.4}  & {86.3} & 14.9 \\
R50-DeAOT-L & \textbf{85.9}  &  \textbf{84.6}  & \textbf{89.4}  & \textbf{80.8}  & \textbf{88.9} & \textbf{22.4} \\
\hline
SwB-AOT-L~\cite{aot}  & {84.5}  &  {84.0}  & {88.8}  & {78.4}  & {86.7} & 9.3 \\
SwB-DeAOT-L & \textbf{86.1}  &  \textbf{85.3}  & \textbf{90.2}  & \textbf{80.4}  & \textbf{88.6} & \textbf{11.9} \\

\bottomrule[1.5pt]
\end{tabular}

\end{subtable}
\begin{subtable}{.45\textwidth}










\caption{DAVIS 2017}\label{tab:full_davis}
\begin{center}
\small
\vspace{-2.3mm}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c c c}
\toprule[1.5pt]
 Methods  & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & FPS \\
\midrule[1pt]
\multicolumn{5}{c}{\textit{Validation 2017 Split}} \\
\midrule[1pt]
AG~\cite{agame}   & 70.0  &  67.2  & 72.7 & 7.1$^\ddag$ \\
FEEL~\cite{feelvos}  &  71.5  &  69.1  & 74.0 & 2.0 \\
SAT~\cite{realtimevos1} &  72.3 & 68.6  & 76.0  & 19.5$^\ddag$ \\
LWL~\cite{LWLVOS} &  81.6  & 79.1  & 84.1 & 2.5$^\ddag$ \\
STM~\cite{spacetime}  &  81.8  & 79.2  & 84.3 & 3.1$^\ddag$ \\
CFBI~\cite{cfbi} &  81.9  & 79.3  & 84.5 & 5.9 \\
SST~\cite{sstvos}  &  82.5  & 79.9  & 85.1 & - \\
EGMN~\cite{EGMN}  &  82.8  & 80.2  & 85.2 & 2.5$^\ddag$ \\
KMN~\cite{KMN} &  76.0  & 74.2  & 77.8 & 4.2$^\ddag$ \\
KMN~\cite{KMN}  &  82.8  & 80.0  & 85.6 & 4.2$^\ddag$ \\
CFBI+~\cite{cfbip}  &  82.9  & 80.1  & 85.7 & 5.6 \\
SST~\cite{sstvos} &  82.5  & 79.9  & 85.1 & - \\
KMN~\cite{KMN}  &  82.8  & 80.0  & 85.6 & 4.2$^\ddag$ \\
CFBI+~\cite{cfbip}  &  82.9  & 80.1  & 85.7 & 5.6 \\
RPCM~\cite{rpcm}  &  83.7  & 81.3  & 86.0 & - \\
HMMN~\cite{hmmn}  &  84.7  & 81.9  & 87.5 & 5.0$^\ddag$ \\
STCN~\cite{cheng2021stcn}  &  85.4  & 82.2  & 88.6 & 24.7$^\star$ \\
\hline
\hline
AOT-T~\cite{aot}  & 79.9 & 77.4 & 82.3 & {51.4} \\
DeAOT-T  & \textbf{80.5} & \textbf{77.7} & \textbf{83.3} & \textbf{63.5} \\
\hline
AOT-S~\cite{aot}  & \textbf{81.3} & \textbf{78.7} & \textbf{83.9} & {40.0} \\
DeAOT-S  & {80.8} & {77.8} & {83.8} & \textbf{49.2} \\
\hline
AOT-B~\cite{aot}  & \textbf{82.5} & \textbf{79.7} & \textbf{85.2} & 29.6 \\
DeAOT-B  & {82.2} & {79.2} & {85.1} & \textbf{40.9} \\
\hline
AOT-L~\cite{aot}  & {83.8} & \textbf{81.1} & {86.4} & 18.7 \\
DeAOT-L  & \textbf{84.1} & {81.0} & \textbf{87.1} & \textbf{28.5} \\
\hline
R50-AOT-L~\cite{aot}  & {84.9} & \textbf{82.3} & {87.5} & 18.0 \\
R50-DeAOT-L  & \textbf{85.2} & {82.2} & \textbf{88.2} & \textbf{27.0} \\
\hline
SwB-AOT-L~\cite{aot}  & {85.4} & {82.4} & {88.4} & 12.1 \\
SwB-DeAOT-L  & \textbf{86.2} & \textbf{83.1} & \textbf{89.2} & \textbf{15.4} \\
\midrule[1pt]
\multicolumn{5}{c}{\textit{Testing 2017 Split}} \\
\midrule[1pt]
FEEL~\cite{feelvos}   &  57.8  &  55.2  & 60.5 & 1.9 \\
STM$^{*}$~\cite{spacetime}  &  72.2  & 69.3  & 75.2 & - \\
CFBI~\cite{cfbi}  &  75.0  & 71.4  & 78.7 & 5.3 \\
CFBI$^{*}$~\cite{cfbi}  &  76.6  & 73.0  & 80.1 & 2.9 \\
STCN~\cite{cheng2021stcn}  &  76.1  & 72.7  & 79.6 & 19.5$^\star$ \\
KMN$^{*}$~\cite{KMN}   &  77.2  & 74.1  & 80.3 & - \\
CFBI+$^{*}$~\cite{cfbip}  &  78.0  & 74.4  & 81.6 & 3.4 \\
HMMN~\cite{hmmn}  &  78.6  & 74.7  & 82.5 & 3.4$^\ddag$ \\
\vspace{0.65mm}
RPCM~\cite{rpcm}  &  79.2  & 75.8  & 82.6 & - \\
\hline
\hline

AOT-T~\cite{aot}  & 72.0 & 68.3 & 75.7 & {51.4} \\
DeAOT-T  & \textbf{73.7} & \textbf{70.0} & \textbf{77.3} & \textbf{63.5} \\
\hline
AOT-S~\cite{aot}  &  73.9  & 70.3 & 77.5 & 40.0 \\
DeAOT-S  & \textbf{75.4} & \textbf{71.9} & \textbf{79.0} & \textbf{49.2} \\
\hline
AOT-B~\cite{aot}   &  75.5  & 71.6 & 79.3 & 29.6 \\
DeAOT-B  & \textbf{76.2} & \textbf{72.5} & \textbf{79.9} & \textbf{40.9} \\
\hline
AOT-L~\cite{aot}   &  \textbf{78.3}  & \textbf{74.3} & \textbf{82.3} & 18.7 \\
DeAOT-L  & {77.9} & {74.1} & {81.7} & \textbf{28.5} \\
\hline
R50-AOT-L~\cite{aot}  & {79.6} & {75.9} & {83.3} & 18.0 \\
R50-DeAOT-L  & \textbf{80.7} & \textbf{76.9} & \textbf{84.5} & \textbf{27.0} \\
\hline
SwB-AOT-L~\cite{aot}  & {81.2} & {77.3} & {85.1} & 12.1 \\
SwB-DeAOT-L  & \textbf{82.8} & \textbf{78.9} & \textbf{86.7} & \textbf{15.4} \\

\bottomrule[1.5pt]

\end{tabular}
\end{center}

\end{subtable}

\end{table}







==> Tables/full_davis2016.tex <==
% \begin{wraptable}[23]{r}{0.43\textwidth}
\begin{table}[t!]
\begin{center}
% \vspace{-13mm}
\vspace{-6.5mm}
\caption{Additional quantitative comparison on DAVIS 2016~\cite{davis2016}.}\label{tab:full_davis2016}

\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c c}
\toprule[1.5pt]
 Methods  & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & FPS \\
\midrule[1pt]
FEEL~\cite{feelvos}   & 81.7  &  81.1 &  82.2 & 2.2 \\
AG~\cite{agame}   &  82.1 & 82.2  & 82.0  & 14.3 \\
SAT~\cite{realtimevos1}   &  83.1 & 82.6  & 83.6  & 39 \\
STM~\cite{spacetime}   &  89.3 & 88.7  & 89.9  & 6.3 \\
CFBI~\cite{cfbi}   & 89.4  & 88.3 & 90.5  & 6.3 \\
CFBI+~\cite{cfbip}   & 89.9  & 88.7 & 91.1  & 5.9 \\
KMN~\cite{KMN}   &  90.5 & {89.5}  & {91.5}  & 8.3 \\
RPCM~\cite{rpcm}  &  90.6  & 87.1  & 94.0 & 5.8 \\
HMMN~\cite{hmmn}   &  90.8 & {89.6}  & {92.0}  & 10.0 \\
STCN~\cite{cheng2021stcn}   &  91.6 & {90.8}  & {92.5}  & 27.2$^\star$ \\
\hline
\hline
AOT-T~\cite{aot}  &  86.8  & 86.1 & 87.4 & {51.4} \\
DeAOT-T  & \textbf{88.9} & \textbf{87.8} & \textbf{89.9} & \textbf{63.5} \\
\hline
AOT-S~\cite{aot}  &  \textbf{89.4}  & \textbf{88.6} & 90.2 & 40.0 \\
DeAOT-S  & {89.3} & {87.6} & \textbf{90.9} & \textbf{49.2} \\
\hline
AOT-B~\cite{aot}  &  89.9  & 88.7 & 91.1 & 29.6 \\
DeAOT-B  & \textbf{91.0} & \textbf{89.4} & \textbf{92.5} & \textbf{40.9} \\
\hline
AOT-L~\cite{aot}  &  {90.4}  & {89.6} & {91.1} & 18.7 \\
DeAOT-L  & \textbf{92.0} & \textbf{90.3} & \textbf{93.7} & \textbf{28.5} \\
\hline
R50-AOT-L~\cite{aot}  &  {91.1}  & {90.1} & {92.1} & 18.0 \\
R50-DeAOT-L  & \textbf{92.3} & \textbf{90.5} & \textbf{94.0} & \textbf{27.0} \\
\hline
SwinB-AOT-L~\cite{aot}  &  {92.0}  & {90.7} & {93.3} & 12.1 \\
SwinB-DeAOT-L  & \textbf{92.9} & \textbf{91.1} & \textbf{94.7} & \textbf{15.4} \\
\bottomrule[1.5pt]

\end{tabular}
\end{center}
% \end{wraptable}
\end{table}

==> Tables/vot.tex <==
\begin{table}[t!]
	\centering
	\caption{The quantitative evaluation on the VOT benchmark, VOT 2020~\cite{}. Sw: SwinB.
	}
\begin{center}
\footnotesize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{l|p{1.6cm}<{\centering} p{2cm}<{\centering}|p{2.2cm}<{\centering} p{2.0cm}<{\centering}|p{2.cm}<{\centering} p{2cm}<{\centering}}
\toprule[1.5pt]
    & RPT~\cite{rpt}                 & MixFormer~\cite{mixformer}          & AOT-S~\cite{aot}                & DeAOT-S              & AOT-B~\cite{aot}                & De-AOT-B             \\
    \midrule[1pt]
EAO &        0.530              &        0.555                   &          0.512            &           \textbf{0.593}                &        0.541              &              \textbf{0.571}                \\
\bottomrule[1.5pt]
\toprule[1.5pt]
    & AOT-L~\cite{aot}                & De-AOT-L             & R50-AOT-L~\cite{aot}                & R50-DeAOT-L             & Sw-AOT-L~\cite{aot}           & Sw-DeAOT-L          \\
    \midrule[1pt]
EAO & 0.574 &   \textbf{0.591}  & 0.569 &  \textbf{0.613}   & 0.586 &    \textbf{0.622}    \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
	
	
\end{table}

==> Tables/youtubevos.tex <==
\begin{table}[t!]
	\centering
	\caption{The quantitative evaluation on multi-object benchmarks, YouTube-VOS~\cite{youtubevos} and DAVIS 2017~\cite{davis2017}. 
	$^{*}$: using 600p videos in inference. $^{\ddag}$: timing extrapolated from single-object speed assuming linear scaling in the number of objects. $^{\star}$: recorded on our device.
	}\label{tab:comparisons}
	
\small
\begin{subtable}[t]{.54\textwidth}
\centering
\caption{YouTube-VOS}\label{tab:youtubevos}
\setlength{\tabcolsep}{3pt}
\vspace{-0.5mm}
\begin{tabular}{lcccccc}
	
\toprule[1.5pt]
            &   &  \multicolumn{2}{c}{Seen}  &    \multicolumn{2}{c}{Unseen} &  \\
\midrule[1pt]
 Method & Avg & $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & fps \\
\midrule[1pt]
\multicolumn{7}{c}{\textit{Validation 2018 Split}} \\
\midrule[1pt]
% STM\pub{ICCV19}~\cite{spacetime}   &  79.4  &  79.7  &  84.2  &  72.8  &  80.9 & - \\
% KMN\pub{ECCV20}~\cite{KMN}  &  81.4  &  81.4  &  85.6  &  75.3  &  83.3 & - \\
% CFBI\pub{ECCV20}~\cite{cfbi} &  81.4  &  81.1  & 85.8  & 75.3  & 83.4 & 3.4 \\
SST~\cite{sstvos} & 81.7  &  81.2  &  -  &  76.0  &  - & - \\
HMMN~\cite{hmmn} & 82.6  &  82.1  &  87.0  &  76.8  &  84.6 & -  \\
CFBI+~\cite{cfbip} &  82.8  &  81.8  & 86.6  & 77.1  & 85.6 & 4.0 \\
STCN~\cite{cheng2021stcn} &  83.0  &  81.9  & 86.5  & 77.9  & 85.7 & 8.4$^\star$ \\
RPCM~\cite{rpcm} &  84.0  &  83.1  & 87.7  & 78.5  & 86.7 & -  \\
\hline
\hline
AOT-T~\cite{aot} & 80.2  &  80.1  & 84.5  & 74.0  & 82.2 & {41.0} \\
DeAOT-T & \textbf{82.0}  &  \textbf{81.6}  & \textbf{86.3}  & \textbf{75.8}  & \textbf{84.2} & \textbf{53.4} \\
\hline
AOT-S~\cite{aot}  & 82.6  &  82.0  & 86.7  & 76.6  & 85.0 & {27.1} \\
DeAOT-S & \textbf{84.0}  &  \textbf{83.3}  & \textbf{88.3}  & \textbf{77.9}  & \textbf{86.6} & \textbf{38.7} \\
\hline
AOT-B~\cite{aot}  & 83.5  &  {82.6}  & 87.5  & {77.7}  & 86.0 & 20.5 \\
DeAOT-B & \textbf{84.6}  &  \textbf{83.9}  & \textbf{88.9}  & \textbf{78.5}  & \textbf{87.0} & \textbf{30.4} \\
\hline
AOT-L~\cite{aot}  & {83.8}  &  {82.9}  & {87.9}  & {77.7}  & {86.5} & 16.0 \\
DeAOT-L & \textbf{84.8}  &  \textbf{84.2}  & \textbf{89.4}  & \textbf{78.6}  & \textbf{87.0} & \textbf{24.7} \\
\hline
R50-AOT-L~\cite{aot}  & {84.1}  &  {83.7}  & {88.5}  & {78.1}  & {86.1} & 14.9 \\
R50-DeAOT-L & \textbf{86.0}  &  \textbf{84.9}  & \textbf{89.9}  & \textbf{80.4}  & \textbf{88.7} & \textbf{22.4} \\
\hline
SwB-AOT-L~\cite{aot}  & {84.5}  &  {84.3}  & {89.3}  & {77.9}  & {86.4} & 9.3 \\
SwB-DeAOT-L & \textbf{86.2}  &  \textbf{85.6}  & \textbf{90.6}  & \textbf{80.0}  & \textbf{88.4} & \textbf{11.9} \\

\midrule[1pt]
\multicolumn{7}{c}{\textit{Validation 2019 Split}} \\
\midrule[1pt]
% CFBI\pub{ECCV20}~\cite{cfbi}  &  81.0  &  {80.6}  & {85.1}  & {75.2}  & {83.0} & 3.4  \\
SST~\cite{sstvos} & 81.8  &  80.9  &  -  &  76.6  &  - & - \\
HMMN~\cite{hmmn} & 82.5  &  81.7  &  86.1  &  77.3  &  85.0 & - \\
CFBI+~\cite{cfbip} &  82.6  &  81.7  & 86.2  & 77.1  & 85.2 & 4.0 \\
STCN~\cite{cheng2021stcn}  &  82.7  &  81.1  & 85.4  & 78.2  & 85.9 & 8.4$^\star$ \\
RPCM~\cite{rpcm} &  83.9  &  82.6  & 86.9  & 79.1  & 87.1 & - \\
\hline
\hline
AOT-T~\cite{aot}  &  79.7  &  79.6  & 83.8  & 73.7  & 81.8 & {41.0} \\
DeAOT-T & \textbf{82.0}  &  \textbf{81.2}  & \textbf{85.6}  & \textbf{76.4}  & \textbf{84.7} & \textbf{53.4} \\
\hline
AOT-S~\cite{aot}  &  82.2 &  81.3  & 85.9  & 76.6  & 84.9 & {27.1} \\
DeAOT-S & \textbf{83.8}  &  \textbf{82.8}  & \textbf{87.5}  & \textbf{78.1}  & \textbf{86.8} & \textbf{38.7} \\
\hline
AOT-B~\cite{aot}  &  83.3 &  {82.4}  & {87.1}  & 77.8  & 86.0 & 20.5 \\
DeAOT-B & \textbf{84.6}  &  \textbf{83.5}  & \textbf{88.3}  & \textbf{79.1}  & \textbf{87.5} & \textbf{30.4} \\
\hline
AOT-L~\cite{aot}  &  {83.7} &  {82.8}  & {87.5}  & {78.0}  & \textbf{86.7} & 16.0 \\
DeAOT-L & \textbf{84.7}  &  \textbf{83.8}  & \textbf{88.8}  & \textbf{79.0}  & \textbf{87.2} & \textbf{24.7} \\
\hline
R50-AOT-L~\cite{aot}  & {84.1}  &  {83.5}  & {88.1}  & \textbf{78.4}  & {86.3} & 14.9 \\
R50-DeAOT-L & \textbf{85.9}  &  \textbf{84.6}  & \textbf{89.4}  & \textbf{80.8}  & \textbf{88.9} & \textbf{22.4} \\
\hline
SwB-AOT-L~\cite{aot}  & {84.5}  &  {84.0}  & {88.8}  & {78.4}  & {86.7} & 9.3 \\
SwB-DeAOT-L & \textbf{86.1}  &  \textbf{85.3}  & \textbf{90.2}  & \textbf{80.4}  & \textbf{88.6} & \textbf{11.9} \\
\bottomrule[1.5pt]
\end{tabular}

\end{subtable}
\begin{subtable}[t]{.45\textwidth}










\caption{DAVIS 2017}\label{tab:davis}
\begin{center}
\vspace{-2.3mm}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c c}
\toprule[1.5pt]
 Method  & Avg & $\mathcal{J}$ & $\mathcal{F}$ & fps \\
\midrule[1pt]
\multicolumn{5}{c}{\textit{Validation 2017 Split}} \\
\midrule[1pt]
%LWL~\cite{LWLVOS}  &  81.6  & 79.1  & 84.1 & 2.5$^\ddag$ \\

SST~\cite{sstvos} &  82.5  & 79.9  & 85.1 & - \\
KMN~\cite{KMN}  &  82.8  & 80.0  & 85.6 & 4.2$^\ddag$ \\
CFBI+~\cite{cfbip}  &  82.9  & 80.1  & 85.7 & 5.6 \\
RPCM~\cite{rpcm}  &  83.7  & 81.3  & 86.0 & - \\
HMMN~\cite{hmmn}  &  84.7  & 81.9  & 87.5 & 5.0$^\ddag$ \\
STCN~\cite{cheng2021stcn}  &  85.4  & 82.2  & 88.6 & 24.7$^\star$ \\
\hline
\hline
AOT-T~\cite{aot}  & 79.9 & 77.4 & 82.3 & {51.4} \\
DeAOT-T  & \textbf{80.5} & \textbf{77.7} & \textbf{83.3} & \textbf{63.5} \\
\hline
AOT-S~\cite{aot}  & \textbf{81.3} & \textbf{78.7} & \textbf{83.9} & {40.0} \\
DeAOT-S  & {80.8} & {77.8} & {83.8} & \textbf{49.2} \\
\hline
AOT-B~\cite{aot}  & \textbf{82.5} & \textbf{79.7} & \textbf{85.2} & 29.6 \\
DeAOT-B  & {82.2} & {79.2} & {85.1} & \textbf{40.9} \\
\hline
AOT-L~\cite{aot}  & {83.8} & \textbf{81.1} & {86.4} & 18.7 \\
DeAOT-L  & \textbf{84.1} & {81.0} & \textbf{87.1} & \textbf{28.5} \\
\hline
R50-AOT-L~\cite{aot}  & {84.9} & \textbf{82.3} & {87.5} & 18.0 \\
R50-DeAOT-L  & \textbf{85.2} & {82.2} & \textbf{88.2} & \textbf{27.0} \\
\hline
SwB-AOT-L~\cite{aot}  & {85.4} & {82.4} & {88.4} & 12.1 \\
SwB-DeAOT-L  & \textbf{86.2} & \textbf{83.1} & \textbf{89.2} & \textbf{15.4} \\
\midrule[1pt]
\multicolumn{5}{c}{\textit{Testing 2017 Split}} \\
\midrule[1pt]
STCN~\cite{cheng2021stcn}  &  76.1  & 72.7  & 79.6 & 19.5$^\star$ \\
KMN$^{*}$~\cite{KMN}   &  77.2  & 74.1  & 80.3 & - \\
CFBI+$^{*}$~\cite{cfbip}  &  78.0  & 74.4  & 81.6 & 3.4 \\
HMMN~\cite{hmmn}  &  78.6  & 74.7  & 82.5 & 3.4$^\ddag$ \\
\vspace{0.65mm}
RPCM~\cite{rpcm}  &  79.2  & 75.8  & 82.6 & - \\
\hline
\hline

AOT-T~\cite{aot}  & 72.0 & 68.3 & 75.7 & {51.4} \\
DeAOT-T  & \textbf{73.7} & \textbf{70.0} & \textbf{77.3} & \textbf{63.5} \\
\hline
AOT-S~\cite{aot}  &  73.9  & 70.3 & 77.5 & 40.0 \\
DeAOT-S  & \textbf{75.4} & \textbf{71.9} & \textbf{79.0} & \textbf{49.2} \\
\hline
AOT-B~\cite{aot}   &  75.5  & 71.6 & 79.3 & 29.6 \\
DeAOT-B  & \textbf{76.2} & \textbf{72.5} & \textbf{79.9} & \textbf{40.9} \\
\hline
AOT-L~\cite{aot}   &  \textbf{78.3}  & \textbf{74.3} & \textbf{82.3} & 18.7 \\
DeAOT-L  & {77.9} & {74.1} & {81.7} & \textbf{28.5} \\
\hline
R50-AOT-L~\cite{aot}  & {79.6} & {75.9} & {83.3} & 18.0 \\
R50-DeAOT-L  & \textbf{80.7} & \textbf{76.9} & \textbf{84.5} & \textbf{27.0} \\
\hline
SwB-AOT-L~\cite{aot}  & {81.2} & {77.3} & {85.1} & 12.1 \\
SwB-DeAOT-L  & \textbf{82.8} & \textbf{78.9} & \textbf{86.7} & \textbf{15.4} \\

\bottomrule[1.5pt]

\end{tabular}
\end{center}

\end{subtable}

\end{table}






